A Framework to Synergize Partial Order Reduction with State Interpolation

We address the problem of reasoning about interleavings in safety verification of concurrent programs. In the literature, there are two prominent techniques for pruning the search space. First, there are well-investigated trace-based methods, collectively known as "Partial Order Reduction (POR)", which operate by weakening the concept of a trace by abstracting the total order of its transitions into a partial order. Second, there is state-based interpolation where a collection of formulas can be generalized by taking into account the property to be verified. Our main contribution is a framework that synergistically combines POR with state interpolation so that the sum is more than its parts.

==> trace.tex <==
In preparing for \por~and \si~to work together,
we now further modify the concept of persistent set
so that it applies for any state sharing the same program point.
The previous definitions apply for a specific state only.

\ignore{
\begin{definition}[Semi-Commutative After A Program Point]
For all $t_1, t_2 \in \mathcal{T}$ and all property $\safety$,
we say $t_1$ \emph{semi-commutes} with $t_2$ \emph{after program point} $\pc$ wrt. 
$\sqsupseteq_\psi$ under the condition $\cons$,
denoted as $\langle \pc, \cons, t_1~\uparrow~t_2, \psi \rangle$ \emph{\myiff}
for all feasible derivation $s_0 \stackrel{\theta}{\Longrightarrow} s$ 
such that $s \equiv \pair{\pc}{\mapstatetoformula{s}}$,
if $\mapstatetoformula{s} \models \cons$ then $t_1$ semi-commutes with $t_2$  after state s 
wrt. $\sqsupseteq_\psi$.
\qed
\end{definition}
}

\begin{definition}[Semi-Commutative After A Program Point]
For a given concurrent program, a safety property $\safety$,
and  $t_1, t_2 \in \mathcal{T}$,
we say $t_1$ \emph{semi-commutes} with $t_2$ 
\emph{after program point} $\pc$ wrt. 
$\sqsupseteq_\psi$ and $\cons$,
denoted as $\langle \pc, \cons, t_1 \uparrow t_2, \psi \rangle$, 
\emph{\myiff}
for all feasible state  $s \equiv \pair{\pc}{\mapstatetoformula{s}}$ 
reachable from the initial state 
$s_0$,
if $\mapstatetoformula{s} \models \cons$ then $t_1$ semi-commutes 
with $t_2$  after state s wrt. $\sqsupseteq_\psi$.
\qed
\end{definition}



\vspace{-2mm}
\newexample{}
Refer back to Ex.~\ref{por:ex:loose} on two loosely coupled processes, we have:

\hspace{5mm}$\forall \pc ~\forall \safety \bullet
\langle \pc, \true, t^{\{1\}}_{1}~\uparrow~t^{\{2\}}_{1}, \psi \rangle$

\hspace{5mm}$\forall \pc ~\forall \safety \bullet
\langle \pc, \true, t^{\{1\}}_{2}~\uparrow~t^{\{2\}}_{1}, \psi \rangle$

\hspace{5mm}$\forall \pc ~\forall \safety \bullet
\langle \pc, \true, t^{\{1\}}_{1}~\uparrow~t^{\{2\}}_{2}, \psi \rangle$ 

\hspace{5mm}$\forall \pc ~\forall \safety \bullet
\langle \pc, \true, t^{\{1\}}_{2}~\uparrow~t^{\{2\}}_{2}, \psi \rangle$.


\begin{definition}[Persistent Set Of A Program Point]
A set $T \subseteq \mathcal{T}$ of transitions schedulable at 
program point $\pc$ is \emph{persistent at $\pc$} under the trace-interpolant 
$\Intpsymbol$ wrt. a property $\safety$ \emph{\myiff}, 
for all feasible derivation $s_0 \stackrel{\theta}{\Longrightarrow} s$ 
such that $s \equiv \pair{\pc}{\mapstatetoformula{s}}$,
if $\mapstatetoformula{s} \models \Intpsymbol$ then  
for all feasible derivations
$s \stackrel{t_1}{\rightarrow} s_1 \stackrel{t_2}{\rightarrow}  s_2 \ldots 
\stackrel{t_{m-1}}{\rightarrow} s_{m-1} \stackrel{t_{m}}{\rightarrow} s_{m}$
including only transitions $t_i \in \mathcal{T}$ and $t_i \not\in T, 1\leq i \leq m$, 
each transition in T semi-commutes with $t_i$ after state $s$ wrt. $\sqsupseteq_\psi$.
\qed
\end{definition}


Assume that $T = \{tp_1, tp_2, \cdots tp_k\}$.
The trace interpolant $\Intpsymbol$ can now be computed as
$\Intpsymbol = \bigwedge \cons_{ji}$ for $1 \leq j \leq k, 1 \leq i \leq m$ 
such that $\langle \pc, \cons_{ji}, tp_j~\uparrow~t_i, \psi \rangle$.

%One can observe that for each program point, 
%if we attempt to find a \emph{smaller} persistent set
%we will indeed strengthen the trace interpolant $\Intpsymbol$. 
%In other words, 
For each program point, it is possible to 
have different persistent sets associated with 
different trace interpolants accordingly. In general,
a state which satisfies a stronger interpolant will have a 
smaller persistent set, and therefore, 
it enjoys more pruning.


\ignore{



\subsection{Approximating the ``semi-commutative'' relation}
\label{sec:por:computing}

In previous parts, we have defined the concepts of 
\emph{trace coverage} and \emph{``semi-commutative''}, 
which give rise to traditional selective search, thus exploit property driven pruning. 
To further relate these concepts to some practical implementation, 
we will hint out \emph{one} possible way to approximate the ``semi-commutative'' relation, 
using state interpolation and precondition propagation.

Assume that we have at hand property $\psi$ and two transitions 
$t_1, t_2 \in \mathcal{T}_{\pc}$. 
We now want to decide whether $t_1$ can semi-commute with $t_2$ 
after program point $\pc$ and wrt. $\sqsupseteq_\psi$. 
In fact, we pose the question as ``with which $\cons$ we can have 
$\aquadruple{\pc}{\cons}{t_1 \uparrow t_2}{\psi}$''.

Abusing notation, for each program point $\pc$ and 
a set of suffix traces $\mathcal{W}$ starting from $\pc$,
i.e., $\mathcal{W} \subseteq \mathcal{W}_{\pc}$, 
let  $\texttt{SI}(\mathcal{W}, \psi)$\footnote{Note that 
with a proper $\mathcal{W}$, information about 
$\pc$ can always be inferred.}
denote the state interpolant such that for all state 
$s \in \typesymbstate$, $s$ is at program point $\pc$,
if $s \models \texttt{SI}(\mathcal{W}, \psi)$ 
then all the derivations from $s$ using the suffices
in $\mathcal{W}$ are safe wrt. $\psi$. 
We also denote 
$\overline{\texttt{SI}}(\mathcal{W}, \psi)$ as the interpolant such that if 
$s \models \overline{\texttt{SI}}(\mathcal{W}, \psi)$, 
all the corresponding derivations are \emph{unsafe}.
Note that $ \overline{\texttt{SI}}(\mathcal{W}, \psi) \models \texttt{SI}(\mathcal{W}, \neg \psi)$. 

If $\mathcal{W}$ contains suffix traces starting from different program point, 
we define $\texttt{SI}(\mathcal{W}, \psi)$ as $\bigwedge_{i = 1..m} \texttt{SI}(\mathcal{W}_i, \psi)$
where $\mathcal{W}_1 \cdots \mathcal{W}_m$ are partitions of $\mathcal{W}$ such that
each set contains only suffices starting from the same program point. 
$\overline{\texttt{SI}}(\mathcal{W}, \psi)$ is defined similarly.

Now we can proceed by finding $\cons_1$ and $\cons_2$ such that:
\begin{align*}
\cons_1 = \overline{\texttt{SI}}(\{t_1 t_2 w_2 | Rng(w_2) \subseteq \mathcal{T}_{\pc} \setminus \{t_1, t_2\}\}, \psi) \\
\cons_2 = \texttt{SI}(\{t_2 t_1 w_2 | Rng(w_2) \subseteq \mathcal{T}_{\pc} \setminus \{t_1, t_2\}\}, \psi)
\end{align*}
We adopt a ``Hoare triple''~\cite{hoare69axiom} notation here.
We need to find $\cons$ such that
for all possible sequences $w_1$, 
$Rng(w_1) \subseteq \mathcal{T}_{\pc} \setminus \{t_1, t_2\}$,
we have
$\{\cons\} w_1 \{\cons_1 \vee \cons_2\}$.

Assume we reach state $s$ at program point $\pc$ through a prefix $\theta$ and
$s \models \cons$. We then have
$\forall w_1 \bullet s \stackrel{w_1}{\Longrightarrow} s_1~implies~s_1 \models \cons_1 \vee \cons_2$.
If it is unsafe before reaching $s_1$, trace coverage is trivially satisfied. Otherwise,
$s_1 \models \cons_1 \vee \cons_2$ implies that $s_1 \models \cons_1 \vee s_1 \models \cons_2$.
If $s_1 \models \cons_1$ then $\forall w_2: \theta w_1 t_1 t_2 w_2$ 
must be unsafe, and therefore
$\forall w_2 \bullet \theta w_1 t_1 t_2 w_2 \sqsupseteq_{\psi} \theta w_1 t_2 t_1 w_2$.
Similarly, if $s_1 \models \cons_2$ then
 $\forall w_2 \bullet \theta w_1 t_2 t_1 w_2$ must be safe.
Again we derive that $\forall w_2 \bullet \theta w_1 t_1 t_2 w_2 
\sqsupseteq_{\psi} \theta w_1 t_2 t_1 w_2$.

}

We emphasize here the obvious challenge of implementing trace interpolation.
This entails obtaining a good estimate of the semi-commutative relation. 
To perform this task generally is non-trivial.
%\footnote{In Appendix-\ref{sec:app:semi}, 
%we hint out one possible approximation technique for this.}.
But importantly, as elaborated in Sec.~\ref{sec:por:experiment}, 
for specific applications, 
based on our formalization of \emph{trace interpolation}, 
it is possible to build \emph{customized} algorithms whereby information
about (property driven) persistent set can be embedded.

We also importantly note here that, 
we can readily use \emph{any} traditional \por~method 
as an approximation of trace interpolation. 
This includes the trivial method 
in which we estimate the ``semi-commutative'' relation as
the traditional independence relation 
(then the trace interpolant is just $\true$). 
Our formalization of trace interpolation makes this possible as 
the proposed concepts are \emph{strictly weaker} than the
corresponding concepts used in traditional \por~methods. 
We stress that even in this setting, 
our combination of state interpolation and \por{} is
in fact \emph{better} than a simple combination of the two underlying
methods (e.g., running each in parallel and seeking the first
termination). Again, we elaborate on this in Sec.~\ref{sec:por:experiment}.

